Meta-Learning for Stochastic Gradient MCMC

Stochastic gradient Markov chain Monte Carlo (SG-MCMC) has become increasingly popular for simulating posterior samples in large-scale Bayesian modeling. However, existing SG-MCMC schemes are not tailored to any specific probabilistic model, even a simple modification of the underlying dynamical system requires significant physical intuition. This paper presents the first meta-learning algorithm that allows automated design for the underlying continuous dynamics of an SG-MCMC sampler. The learned sampler generalizes Hamiltonian dynamics with state-dependent drift and diffusion, enabling fast traversal and efficient exploration of neural network energy landscapes. Experiments validate the proposed approach on both Bayesian fully connected neural network and Bayesian recurrent neural network tasks, showing that the learned sampler out-performs generic, hand-designed SG-MCMC algorithms, and generalizes to different datasets and larger architectures.

==> Training.tex <==
\section{Cross-Chain In-Chain Training}
We have designed the efficient parametrization of pre-conditioning matrix in previous section. The remaining challenge is to design the procedure to train the parameters $\phi_D$ and $\phi_Q$. Specifically, we want the trained sampler to have faster convergence and low bias. One possible scheme is to use adversarial training given that real samples are available, or bootstrap method can be used \citep{song2017nice,arjovsky2017wasserstein}. There exists another objective to minimize the lag-one autocorrelation which is equivalent to minimize the expected squared jumped distance \citep{levy2017generalizing,pasarica2010adaptively}. However, the Adversarial training uses GAN-based approach which will be infeasible in very high dimensional problems, whereas expected squared jump distance does not explicitly take the sampling bias and convergence speed into account. Therefore, we need to design a new schemes. One possible objective is to minimize the KL divergence between the distribution formed by Stochastic Dynamics and targeted one. However, the distribution of the dynamics controlled by Eq.\ref{eq:Continuous SDE} are characterized by Fokker-Planck equation. This is not easily solvable for general case. To mediate this problem, we adopt recent advances in training implicit models, specifically the gradient estimator for implicit models \citep{li2017stein}.
\subsection{ELBO}
In the context of variational inference, minimizing the KL divergence between candidate distribution $q_{\phi}(\pmb{\theta}|\mathcal{D})$ and targeted posterior $p(\pmb{\theta}|\mathcal{D})$ is equivalent to maximizing the ELBO:
\begin{equation}
\begin{split}
\mathcal{L}_{\text{VI}}(q)&=\mathbb{E}_{q}[\log p(\pmb{x},\pmb{\theta})]+\mathbb{H}[q_{\phi}(\pmb{\theta}|\pmb{x})]\\
&=\mathbb{E}_{q}[-U(\pmb{\theta})]+\mathbb{H}[q_{\phi}(\pmb{\theta}|\pmb{x})]
\end{split}
\label{eq: ELBO}
\end{equation}
During training, we are only interested in the gradient of $\mathcal{L}_{\text{VI}}$ w.r.t $\phi$. Using re-parametrization tricks (CITE), we have $\pmb{\theta}\sim q_{\phi}(\pmb{\theta}|\mathcal{D}) \Leftrightarrow \pmb{\epsilon}\sim \pi(\pmb{\epsilon}), \pmb{\theta}=\pmb{f}_{\phi}(\pmb{\epsilon},\pmb{\mathcal{D}})$, where in our case, $\pmb{f}_{\phi}$ are stochastic update equation defined as Eq.\ref{eq: update rule}. Thus, the gradient of the parameter $\phi$ can be computed by a sum of the path gradient of the first term ($\mathbb{E}_{\pi}[\nabla_{\pmb{f}}\log p(\pmb{x},\pmb{f}(\pmb{\epsilon},\pmb{x}))^T\nabla_{\phi}\pmb{f}(\pmb{\epsilon},\pmb{x})]$) and the gradient of the entropy term $\nabla_{\phi}\mathbb{H}[q_{\phi}(\pmb{\theta}|\pmb{x})]=-\mathbb{E}_{\pi}[\nabla_{\pmb{f}}\log q_{\phi}(\pmb{f}_{\phi}(\pmb{\epsilon},\pmb{x})|\pmb{x})\nabla_{\phi}\pmb{f}_{\phi}(\pmb{\epsilon},\pmb{x})]$\citep{roeder2017sticking,li2017stein}. $\nabla_{\phi}\pmb{f}_{\phi}(\pmb{\epsilon},\pmb{x})$ can be handled by back-propagating through the Markov Chain, whereas $\nabla_{\pmb{f}}\log q_{\phi}(\pmb{f}_{\phi}(\pmb{\epsilon},\pmb{x}))$ requires an gradient estimator. \medskip\\
\cite{li2017stein} proposed an gradient estimator based on inverting the kernelized Stein discrepancy (KSD) \citep{liu2016kernelized,chwialkowski2016kernel}. To be specific, for a given set of samples $\{\pmb{\theta}_n\}_{n=1}^N$, we define a matrix form of the approximated collected gradients as $\pmb{G}:\approx(\nabla_{\pmb{\theta}_1}\log(q(\pmb{\theta}_1)),\ldots,\nabla_{\pmb{\theta}_N}\log(q(\pmb{\theta}_N)))^T$. We also define a kernel function $\mathcal{K}(\cdot,\cdot)$, and the corresponding kernel matrix $\pmb{K}$. In this paper, we choose RBF kernel and select the bandwidth using median heuristic. Thus, \cite{li2017stein} showed that by using ridge regression, one can obtain the estimated $\pmb{G}$ that minimize KSD:
\begin{equation}
\pmb{G}_{\text{Stein}}=-(\pmb{K}+\eta\pmb{I})^{-1}\langle\nabla,\pmb{K}\rangle
\label{eq:Gradient Estimator}
\end{equation}
where $\eta$ is the regularization term. 

\subsection{Cross-Chain Training}
First, let's consider the distribution represented by the discretized update equation. Typically, the marginal distribution $q_t(\pmb{\theta}|\mathcal{D})$ is intractable at time t, since it involves both intractable proposal distribution  $q(\pmb{\theta}_t|\pmb{\theta}_{t-1},\mathcal{D})$ and integration over all possible paths. Thus, we can use Monte Carlo methods to approximate $q_t$ using samples $\{\pmb{\theta}\}_{n=1}^N\sim q_t$. We can achieves this by running multiple parallel Markov Chains and take samples across the chain. For fast convergence, this can be interpreted as $q_t$ is closed to target posterior $p(\pmb{\theta}|\mathcal{D})$ when $t$ is small. In the cross-chain settings, we run $N$ parallel Markov Chains. First we can initialize the samples by drawing $\{\pmb{\theta}^0\}_{n=1}^N \sim \pi(\pmb{\epsilon})$. Then, simulate the update rule $\pmb{f}_{\phi}$
\begin{equation}
\{\pmb{\theta}^{t+1}\}_{n=1}^N=\pmb{f}_{\phi}(\{\pmb{\theta}^t\}_{n=1}^N,\mathcal{D})\;\;,\;\;\; \hat{q}_t=\frac{1}{N}\sum_{n=1}^N{\delta_{\pmb{\theta}^t_n}}
\end{equation}
Thus, the corresponding ELBO at time t will be 
\begin{equation}
\mathcal{L}_{\text{VI}}^t(\{\pmb{\theta}^t\}_{n=1}^N)=\frac{1}{N}\sum_{n=1}^N{\log p(\mathcal{D},\pmb{\theta}^t_{n})}-\frac{1}{N}\sum_{n=1}^N{\log q(\pmb{\theta}_n^t|\mathcal{D})}
\end{equation}
Thus, we do not use thinning samples, the cross-chain training objective for total running time $T$ is 
\begin{equation}
\mathcal{L}_{\text{cross}}=\frac{1}{T}\sum_{t=1}^T{\mathcal{L}_{\text{VI}}^t(\{\pmb{\theta}^t\}_{n=1}^N)}
\label{eq: Objective Cross Chain}
\end{equation}
By minimizing this objective, we can expect the trained sampler will have a faster convergence, especially at the early times of the Markov Chain. This objective also takes the sampler bias into account, because when KL is minimized, two distributions will match. \medskip\\
During back-propagating through the Markov chain, we also apply stop gradients. We manually stop the gradient pass through the energy function $U(\pmb{\theta})$ and $\nabla_{\pmb{\theta}}(U(\pmb{\theta}))$. This will stabilize the training and avoid higher order gradient computation. Also, we argue that for better generalization, $\pmb{Q}$ and $\pmb{D}$ should not rely on higher order information of the distribution. We refer the reader to Appendix for detailed back-propagation scheme. 
\subsection{Optional: In-Chain Training}
Cross-Chain training objective only considers the discrepancy between $q_t$ and targeted distribution for specific time t. However, even the Cross-Chain objective is minimized, the resulting sampler does not necessary achieve good mixing because the resulting dynamics across time is not considered. For example, in extreme cases, our sampler are just fixed samples from the targeted distribution. Therefore, this sampler can achieve very low Cross-Chain objective, but clearly, this is a very poor sampler due to zero exploration. In practice, the above situation rarely happens, therefore, and whether the In-chain loss is useful depends on how we choose posterior samples for evaluation. In this paper, for high dimensional problem, we will take samples across chains. Thus, we consider the following In-chain training as optional. \medskip\\
First, we can sub-sample $K$ the parallel chains across time $\{\pmb{\theta}^t_k\}_{t=1}^T\sim \{\{\pmb{\theta}_n^t\}_{n=1}^N\}_{t=1}^T$, further, we define $q_{T,K}(\pmb{\theta}|\mathcal{D})$ as the distribution represented by sub-sampled Markov Chains. The samples from the sub-sampled chains can be considered $\{\{\pmb{\theta}_k^t\}_{k=1}^K\}_{t=1}^T\sim q_{T,K}(\pmb{\theta}|\mathcal{D})$. The In-chain training objective is 
\begin{equation}
\mathcal{L}_{\text{In-chain}}(\{\{\pmb{\theta}_k^t\}_{k=1}^K\}_{t=1}^T)=\frac{1}{TK}\sum_{t=1}^T\sum_{k=1}^K{\log p(\mathcal{D},\pmb{\theta}_{k}^t)-\log q_{T,K}(\pmb{\theta}_k^t|\mathcal{D})}
\end{equation}
For the extreme cases mentioned above, the entropy term $\sum_{t=1}^T\sum_{k=1}^K{-\log q_{T,K}(\pmb{\theta}_k^t|\mathcal{D})}$ will result in high KL divergence due to concentrated samples across time. The difference of these two objectives are mainly the entropy term.\medskip\\


==> meta_sampler.tex <==
\section{Meta learning for SG-MCMC}

Our aim is to design an appropriate parameterization of $\pmb{D}(\pmb{z})$ and $\pmb{Q}(\pmb{z})$, so that the sampler can be trained on small tasks with a meta-learning procedure, and generalize to more complicated densities in high dimensions. For simplicity, in the this paper, we only augment the space by introducing one auxiliary variable $\pmb{p}$ called momentum (similar to SGHMC \citep{chen2014stochastic}), although generalization to temperature variable augmentation is fairly straight-forward. Thus, the Hamiltonian is defined as $H(\pmb{z})=U(\pmb{\theta})+\frac{1}{2}\pmb{p}^T\pmb{p}$.

\subsection{Efficient parameterization of SG-MCMC with neural networks}

One difficulty of generalization is that for complicated problems, the dimensionality of $\pmb{\theta}$ will be at least tens of thousands. Thus, training and applying full $\pmb{D}(\pmb{z})$ and $\pmb{Q}(\pmb{z})$ matrix can cause huge computational burden. A simple solution of this difficulty is to use diagonal matrix, where a typical strategy utilities \emph{coordinate-wise parameterization}, i.e. $\pmb{D}(\pmb{z}) = \text{diag}(f_{\phi}(z_1), f_{\phi}(z_2), ..., f_{\phi}(z_{2D}))$ where $f_{\phi}(\cdot)$ is a simple neural network shared across dimensions. Therefore, the dimension generalization can simply be done by copying the functions for each new dimensions. It is a popular recipe deployed by many recent proposals of meta-learned optimizers \citep{andrychowicz2016learning}.
% 

However, this diagonalization decouples the correlations between different dimensions and also the different function output of the each dimension will be controlled by using different inputs. Thus, the selection of inputs to these functions will be crucial. This directly determines how much information about the distribution can be accessed by the function. We will discuss this in the later section.\medskip\\
Based on the previous discussion, we define the preconditioning matrix as follows:
\begin{equation}
\begin{split}
\pmb{Q}&=\left[\begin{array}{cc}
\pmb{0}&-\pmb{Q}_{f}\\
\pmb{Q}_f&\pmb{0}
\end{array}\right]\;,\;\pmb{Q}_f=\text{diag}[f_{\phi_Q}(\cdot)]\\
\pmb{D}&=\left[\begin{array}{cc}
\pmb{0}&\pmb{0}\\
\pmb{0}&\pmb{D}_f
\end{array}
\right]\;,\;\pmb{D}_f=\text{diag}[f_{\phi_D}(\cdot)]
\end{split}
\label{eq: Def of D and Q}
\end{equation}
where $f_{\phi_Q}$ and $f_{\phi_D}$ are two functions with corresponding parameters $\phi_Q$ and $\phi_D$. Notice that according to \textbf{Theorem} \ref{thm: stationary distribution}, $\pmb{Q}$ matrix by design is a \textit{skew-symmetric} matrix and as long as the function $f_{\phi_D}$ only outputs non-negative values, $\pmb{D}$ matrix is \textit{positive semi-definite}. Thus, the stationary distribution for the stochastic dynamics with these two preconditioning matrix will be $p^s(\pmb{\theta})\propto\exp(-U(\pmb{\theta}))$. \medskip \\
The intuition behind this design is simple, but before, we should examine the role of each precondition matrix. Based on Eq.\ref{eq:Continuous SDE} and \ref{eq: Def of D and Q}, matrix $\pmb{Q}$ mainly controls the drift forces introduced by the \textit{energy gradient} $\nabla_{\pmb{\theta}}{U(\pmb{\theta})}$ or \textit{stochastic gradient} $\nabla_{\pmb{\theta}}{\tilde{U}(\pmb{\theta})}$. In this paper, we will assume the gradient is noisy and the noise is Gaussian $\nabla_{\pmb{\theta}}{\tilde{U}(\pmb{\theta})}=\nabla_{\pmb{\theta}}{U(\pmb{\theta})}+\mathcal{N}(\pmb{0},\pmb{B}(\pmb{\theta}))$. Therefore, based on the complete framework, additional friction term should be added to counterbalance the noise effect. Note that the only stochasticity appears at the stochastic gradient. This corresponds to the update for momentum term. Therefore, the friction is only needed for momentum. Matrix $\pmb{D}_f$ controls the amount of frictions and injected noises to the momentum. Therefore, a practical discretization update rule with step size $\epsilon$ is 
\begin{equation}
\begin{split}
\pmb{\theta}_{t+1}&=\pmb{\theta}_t+\epsilon\pmb{Q}_f(\pmb{z}_{t})\pmb{p}_t+\epsilon\Gamma_{\pmb{\theta}}(\pmb{z}_t)\\
\pmb{p}_{t+1}&=\pmb{p}_t-\epsilon\pmb{Q}_f(\pmb{z}_t)\nabla{{U}(\pmb{\theta})}-\epsilon\pmb{D}_f(\pmb{z}_t)\pmb{p}_t+\epsilon\Gamma_{\pmb{p}}(\pmb{z}_t)+\mathcal{N}(\pmb{0},2\epsilon\pmb{D}_f-\epsilon^2\pmb{Q}_f^2\hat{\pmb{B}}(\pmb{\theta}_t))+\mathcal{N}(\pmb{0},\epsilon^2\pmb{Q}_f^2\pmb{B}(\pmb{\theta}))
\end{split}
\label{eq: update rule}
\end{equation}
where $\hat{\pmb{B}}(\pmb{\theta})\approx \pmb{B}(\pmb{\theta})$ is the approximation to the covariance matrix of mini-batch noise.
Ideally, if $\hat{\pmb{B}}=\pmb{B}$, the momentum update will simply be $\triangle \pmb{p}=-\epsilon\pmb{Q}_f\nabla{U(\pmb{\theta})}-\epsilon\pmb{D}_f\pmb{p}_t+\epsilon\Gamma_{\pmb{p}}+\mathcal{N}(\pmb{0},\epsilon\pmb{D}_f)$. This is exactly the discretized version of SDE defined in Eq.\ref{eq:Continuous SDE} and \ref{eq:Gamma def}, thus, when $\epsilon\to 0$, this update equation will maintain the correct stationary distribution $\exp(-U(\pmb{\theta}))$ according to the complete framework. In practice, accurate estimation of mini-batch sampling noise is infeasible, one can use empirical Fisher information for the estimation as \citep{ahn2012bayesian}. Further, if $\epsilon\to 0$, the mini-batch noise term diminishes more quickly than injected noise covariance $2\epsilon\pmb{D}_f$, thus, the dynamics is again governed by SDE from Eq.\ref{eq:Gamma def}.\medskip\\
Further, we observe that $\pmb{D}_f$ matrix should also account for the pre-conditioning effect introduced by $\pmb{Q}_f$. For example, when the magnitude of $\pmb{Q}_f$ is large,due to the infeasibility of computing acceptance rate of MH step, we can only prevent the divergence by introducing a larger momentum frictions. Therefore, we can simply re-define $\pmb{D}_f$ as 
\begin{equation}
\pmb{D}_f=\pmb{Q}_f^2\times constant+\text{diag}[f_{\phi_D}(\cdot)]
\label{eq: Df}
\end{equation}
where the constant can be heuristically chosen to be roughly the same as SGHMC friction.
\subsection{State Dependent Input}
In order to generalize to higher dimension problems, another crucial factor is how much information the meta sampler can access. For example, one can use geometric information about the distribution like Riemannian based sampler(CITE), or the Fisher information matrix (CITE). Other methods uses like preconditioning SGLD (P-SGLD) uses moving averages technique to estimate second moments information. However, this method in fact is based on higher order Markov Chains, which is not included in the complete framework. To keep this in mind, we only discuss the first order Markov method in this paper. On the other hand, richer information comes with a high computational cost, especially in this complete framework, the $\Gamma(\pmb{z})$ matrix. Thus, the input to $f_{\phi_Q}$ and $f_{\phi_D}$ should be carefully chosen such that they contain useful information about distributions but without introducing high computational cost of $\Gamma(\pmb{z})$ matrix. \medskip\\
Based on the previous discussion, $\pmb{Q}$ matrix mainly controls the drift of the dynamics. One useful information is the $U(\pmb{\pmb{\theta}})$ which can be seen as the 'height' of the $\pmb{\theta}$ at the energy landscape. This information can be used to determine if the samples have reached the high density region. The corresponding $\Gamma$ term will require the $\nabla_{\theta}U(\pmb{\theta})$, which is also needed for updating equations Eq.\ref{eq: update rule}. Thus, this does not introduce extra computations. History information can also be very useful (CITE Learning squared). However, due to the constraints of first order Markov chain, we can not use arbitrary history. Momentum $p_i$ is the accumulated gradient which is also the augmented variable in state space. Thus, including it does not violated the Markov property but also provides the 'velocity' of the samples. This information only introduce a first order gradient $\nabla_{p_i}f_{\phi_Q}(U(\pmb{\theta},p_i))$ for $\Gamma$ which can be efficiently computed using Automatic differentiation. In fact, $\nabla_{\pmb{\theta}}U(\pmb{\theta})$ will be more useful to determine whether the sampler has reached the local optimum than $U(\pmb{\theta})$, however, introducing this will requires the diagonal of Hessian for $\Gamma(\pmb{z})$ which is not feasible for high dimensional problems. One way to solve this is to use Fisher information matrix or finite differences for estimation, but we do not consider this approach here. In practice, we may consider put an offset to $\pmb{Q}$ to avoid the too-small step size. Thus, the parametrization of the $\pmb{Q}_f$ is 
\begin{equation}
\pmb{Q}_f=\text{diag}[\pmb{f}_{\phi_Q}]\;\;\;\;\; \pmb{f}_{\phi_Q,i}=constant+f_{\phi_Q}(U(\pmb{\theta}),p_i) 
\label{eq:Q param}
\end{equation}
The expected behavior of $\pmb{Q}$ matrix is that it will output a large value when $U(\pmb{\theta})$ is high for fast traverse through low density region and $p_i$ will 'fine-tune' this output.\medskip\\
$\pmb{D}$ matrix is responsible for friction term and injected noise. This term is crucial to counter the effect of the mini-batch noise. Similarly, we can introduce the same input of $\pmb{Q}$ to $\pmb{D}$. In addition, we can now add gradient $\nabla_{\theta_i}U(\pmb{\theta})$ as the input. Due to the fact that only the bottom right of $\pmb{D}$ matrix is non-zero, thus, we can avoid the Hessian computation for $\Gamma$ matrix. Thus, the parametrization is 
\begin{equation}
\pmb{D}_f=\pmb{Q}_f^2\times constant+\text{diag}[\pmb{f}_{\phi_D}]\;\;\;\;\;\pmb{f}_{\phi_D,i}=f_{\phi_D}(U(\pmb{\theta}),p_i,\nabla_{\theta_i}U(\pmb{\theta}))
\label{eq:D param}
\end{equation}
\subsubsection{Input Pre-processing}
In order to generalize to higher dimensions, certain input pre-processing are needed. First, we can determine the scale of the momentum $p_i$ and $\nabla_{\theta_i}U(\pmb{\pmb{\theta}})$ by random initializing $f_{\phi_D}$ and $f_{\phi_Q}$ and running sampler for several iterations. Then re-scale these inputs to roughly the same scale. From Eq.\ref{eq:U}, this value will scale up linearly with dimensions, thus, we need to properly scale this the energy term by the ratio of training dimension and generalization dimension.  
\subsubsection{Finite Difference $\Gamma(\pmb{z})$}
Although the extra computational burden of $\Gamma$ matrix is feasible due to high parallelization power of GPU, we can still further cut this cost through replacing exact gradient computation by finite difference approximations. The basic idea is to compute the difference of $\pmb{Q}$ and $\pmb{D}$ between previous and current state value and then divided by the state difference. We refer the reader to Appendix for details.

